Ion native variational ansatz for quantum approximate optimization

Variational quantum algorithms involve training parameterized quantum circuits using a classical co-processor. An important variational algorithm, designed for combinatorial optimization, is the quantum approximate optimization algorithm. Realization of this algorithm on any modern quantum processor requires either embedding a problem instance into a Hamiltonian or emulating the corresponding propagator by a gate sequence. For a vast range of problem instances this is impossible due to current circuit depth and hardware limitations. Hence we adapt the variational approach -- using ion native Hamiltonians -- to create ansatze families that can prepare the ground states of more general problem Hamiltonians. We analytically determine symmetry protected classes that make certain problem instances inaccessible unless this symmetry is broken. We exhaustively search over six qubits and consider upto twenty circuit layers, demonstrating that symmetry can be broken to solve all problem instances of the Sherrington-Kirkpatrick Hamiltonian. Going further, we numerically demonstrate training convergence and level-wise improvement for up to twenty qubits. Specifically these findings widen the class problem instances which might be solved by ion based quantum processors. Generally these results serve as a test-bed for quantum approximate optimization approaches based on system native Hamiltonians and symmetry protection.

==> data_clt.tex <==
\subsection{Collecting data (CLT bounds)}

In variational quantum computation, we seek to calculate the expected values of Pauli strings. For a single qubit we repeatedly evaluate the circuit and perform a projective measurement in the $X$, $Y$ or $Z$ basis. We then estimate the probability $p$ of obtaining the ``0'' result. The expected value is then
\begin{equation}\label{eq:h_of_p}
    \hat{h}_\psi = \bra{\psi}H\ket{\psi} = 2\hat{p} - 1.
\end{equation}

Since the measurement statistics is binomial, the estimator variance is $\mathbb{V}(\hat{p})=p(1-p)/n$ for $p$ and $\mathbb{V}(\hat{h}_\psi)=4\mathbb{V}(\hat{p})=(1-h_\psi^2)/n$ for $h_\psi$. Here $n$ is the number of circuit evaluations. From the central limit theorem, it follows that
\begin{equation}\label{eq:clt_error}
    \mathbb{P}\left(|\hat{h}_\psi-h_\psi| \geq \sqrt{D_H}q_{\alpha/2}\right) = \alpha,
\end{equation}
where $q_{\alpha/2}$ is the $(1-\alpha/2)$\textit{th} quantile of the standard normal distribution. Thus, the required sample size to get the estimation accuracy at least $\delta$ with probability $1 - \alpha$ is
\begin{equation}\label{eq:sample_bound}
    n = \left(\frac{q_{\alpha/2}}{\delta}\right)^2(1-h_\psi^2),
\end{equation}
which is bounded by $n=(q_{\alpha/2}/\delta)^2$ for the worst case of $h_\psi=0$.



==> gates-report-2021.tex <==


\section{Toffoli} 

A $k-$controlled Toffoli gate [] applies a reversible variant of the logical $k-AND$ function. Written in matrix form the $k-$ Toffoli is given as 

$$ C_{k}^{̱\underline{m}} = \mathbb{1}_{k} \oplus X = \Bigl[\sum _{\underline{m }  \in  \{0,1\}^{n}}\ketbra{\underline{m }}{\underline{m }}
\Bigr] \oplus  X $$

where
${\underline{m}$ is a vector of indices which we consider equivalently as qubit labels, $m_1,m_2,\ldots, m_k$ and $X$ represents the sigma matrix
 $$X=\sigma_X=\ketbra{0}{1}+\ketbra{1}{0}.$$

The $k-$Toffoli is centrally applied 
in a multitude of settings including Grover search and QAOA penalty function realisations.

The $k-$ Toffoli is locally equivalent to the $k-$ controlled $Z$ gate $(k-C_Z$ or $C_{Z}^{\underline{m}})$ as

$$[\mathbb{1}_{k} \otimes H]  C_{x}^{\underline{m}}[\mathbb{1}_{k} \otimes H]=C_{z}^{\underline{m}$$

And so for any $g \in U(2)$ such that $g=UZU^{\dagger}$ for unitary $U$, and $Z=\ketbra{0}{0}-\ketbra{1}{1},$ one readily creates a $k-$controlled $g-$ gate, $C_{g}^{\underline{m}.$

The $k-$controlled gate applies a $k+1$ body interaction. As such, ample effort has been spent on factoring the $k-$Toffoli into a product of $2-$body gates, imposing various restrictions on the gates employed.

The prototypical factorization for the $2-Toffoli$ is as follows:


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1, baseline=(XXXX.south) ]
\path (0,216);\path (560,0);\draw    ($(current bounding box.center)+(0,0.3em)$) node [anchor=south] (XXXX) {};
%Straight Lines [id:da011133986739978008] 
\draw    (16.67,44.5) -- (316.67,44.5) ;
%Straight Lines [id:da2237132108077906] 
\draw    (14.67,81.5) -- (296.67,80.5) ;
%Straight Lines [id:da25155470138670655] 
\draw    (15.67,119.5) -- (72.67,118.5) ;
%Flowchart: Process [id:dp6762548921630998] 
\draw   (72.67,106.5) -- (98.67,106.5) -- (98.67,133.5) -- (72.67,133.5) -- cycle ;
%Straight Lines [id:da49068056217683154] 
\draw    (85.67,80.5) -- (85.67,106.5) ;
%Straight Lines [id:da5018376686020041] 
\draw    (97.67,119.5) -- (128.67,119.5) ;
%Flowchart: Process [id:dp03960045056492656] 
\draw   (127.67,106.5) -- (153.67,106.5) -- (153.67,133.5) -- (127.67,133.5) -- cycle ;
%Straight Lines [id:da41785901292756256] 
\draw    (153.67,119.5) -- (231.67,119.5) ;
%Flowchart: Process [id:dp1385965750202962] 
\draw   (232.67,104.5) -- (258.67,104.5) -- (258.67,131.5) -- (232.67,131.5) -- cycle ;
%Straight Lines [id:da012059818160674363] 
\draw    (140.67,44.5) -- (140.67,106.5) ;
%Flowchart: Or [id:dp09139752874947638] 
\draw   (181.83,81.25) .. controls (181.83,75.17) and (186.53,70.25) .. (192.33,70.25) .. controls (198.13,70.25) and (202.83,75.17) .. (202.83,81.25) .. controls (202.83,87.33) and (198.13,92.25) .. (192.33,92.25) .. controls (186.53,92.25) and (181.83,87.33) .. (181.83,81.25) -- cycle ; \draw   (181.83,81.25) -- (202.83,81.25) ; \draw   (192.33,70.25) -- (192.33,92.25) ;
%Straight Lines [id:da2816459585703701] 
\draw    (192,44.75) -- (192.33,81.25) ;
%Straight Lines [id:da9921968211681558] 
\draw    (245,80) -- (245.67,104.5) ;
%Flowchart: Or [id:dp545210762971136] 
\draw   (274.83,80.25) .. controls (274.83,74.17) and (279.53,69.25) .. (285.33,69.25) .. controls (291.13,69.25) and (295.83,74.17) .. (295.83,80.25) .. controls (295.83,86.33) and (291.13,91.25) .. (285.33,91.25) .. controls (279.53,91.25) and (274.83,86.33) .. (274.83,80.25) -- cycle ; \draw   (274.83,80.25) -- (295.83,80.25) ; \draw   (285.33,69.25) -- (285.33,91.25) ;
%Straight Lines [id:da8457208939255518] 
\draw    (285,44.75) -- (285.33,81.25) ;
%Straight Lines [id:da7179881166636866] 
\draw    (259.67,119.5) -- (316.67,119.5) ;
%Straight Lines [id:da010024502409413438] 
\draw    (296.67,80.5) -- (319.5,80.5) ;
%Straight Lines [id:da26133815380113457] 
\draw    (356.67,46.5) -- (533.67,47.5) ;
%Straight Lines [id:da39887432069570283] 
\draw    (357.67,81.5) -- (534.67,82.5) ;
%Straight Lines [id:da13504984765686023] 
\draw    (359,119.5) -- (536,120.5) ;
%Flowchart: Or [id:dp07595341562927849] 
\draw   (437,120) .. controls (437,113.92) and (441.7,109) .. (447.5,109) .. controls (453.3,109) and (458,113.92) .. (458,120) .. controls (458,126.08) and (453.3,131) .. (447.5,131) .. controls (441.7,131) and (437,126.08) .. (437,120) -- cycle ; \draw   (437,120) -- (458,120) ; \draw   (447.5,109) -- (447.5,131) ;
%Straight Lines [id:da2769262619904933] 
\draw    (447.17,47) -- (447.5,109) ;
%Straight Lines [id:da5204091395657096] 
\draw    (330.67,76.5) -- (344.67,76.5) ;
%Straight Lines [id:da9525005916225495] 
\draw    (330.67,85.5) -- (344.67,85.5) ;
%Shape: Ellipse [id:dp5441841411686901] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (82,81.75) .. controls (82,79.13) and (83.94,77) .. (86.33,77) .. controls (88.73,77) and (90.67,79.13) .. (90.67,81.75) .. controls (90.67,84.37) and (88.73,86.5) .. (86.33,86.5) .. controls (83.94,86.5) and (82,84.37) .. (82,81.75) -- cycle ;
%Shape: Ellipse [id:dp6753954640053548] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (137,44.75) .. controls (137,42.13) and (138.94,40) .. (141.33,40) .. controls (143.73,40) and (145.67,42.13) .. (145.67,44.75) .. controls (145.67,47.37) and (143.73,49.5) .. (141.33,49.5) .. controls (138.94,49.5) and (137,47.37) .. (137,44.75) -- cycle ;
%Shape: Ellipse [id:dp5528514161249112] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (188,44.75) .. controls (188,42.13) and (189.94,40) .. (192.33,40) .. controls (194.73,40) and (196.67,42.13) .. (196.67,44.75) .. controls (196.67,47.37) and (194.73,49.5) .. (192.33,49.5) .. controls (189.94,49.5) and (188,47.37) .. (188,44.75) -- cycle ;
%Shape: Ellipse [id:dp23136263798259682] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (241,80.75) .. controls (241,78.13) and (242.94,76) .. (245.33,76) .. controls (247.73,76) and (249.67,78.13) .. (249.67,80.75) .. controls (249.67,83.37) and (247.73,85.5) .. (245.33,85.5) .. controls (242.94,85.5) and (241,83.37) .. (241,80.75) -- cycle ;
%Shape: Ellipse [id:dp39956405493933134] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (281,44.75) .. controls (281,42.13) and (282.94,40) .. (285.33,40) .. controls (287.73,40) and (289.67,42.13) .. (289.67,44.75) .. controls (289.67,47.37) and (287.73,49.5) .. (285.33,49.5) .. controls (282.94,49.5) and (281,47.37) .. (281,44.75) -- cycle ;
%Shape: Ellipse [id:dp765760118097758] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (443,81.75) .. controls (443,79.13) and (444.94,77) .. (447.33,77) .. controls (449.73,77) and (451.67,79.13) .. (451.67,81.75) .. controls (451.67,84.37) and (449.73,86.5) .. (447.33,86.5) .. controls (444.94,86.5) and (443,84.37) .. (443,81.75) -- cycle ;
%Shape: Ellipse [id:dp8810538871866143] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (443,46.75) .. controls (443,44.13) and (444.94,42) .. (447.33,42) .. controls (449.73,42) and (451.67,44.13) .. (451.67,46.75) .. controls (451.67,49.37) and (449.73,51.5) .. (447.33,51.5) .. controls (444.94,51.5) and (443,49.37) .. (443,46.75) -- cycle ;
% Text Node
\draw (79,110.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {V};
% Text Node
\draw (134,110.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {V};
% Text Node
\draw (234.67,106) node [anchor=north west][inner sep=0.75pt]   [align=left] {V$\displaystyle ^{\dagger }$};
\end{tikzpicture}

This is derived as follows:

$a\oplus b=a+b-2ab, a,b \in \mathbb{B}.$

Let $V=\sqrt{X}$ then

$$X^{ab}=[V^2]^{ab}=V^aV^b[V^{-1}]^{a\oplus b}$$

From which we arrive immediately at the circuit in $(1).$

This has several generalizations. Firstly we might let $\Tilde{c}$ be an index vector $\Tilde{c}=(c_1,\ldots,c_q)$ and then 

$2ab\tilde{c}=a\Tilde{c}+b\Tilde{c}-[a\oplus b].\Tilde{c}$ admits the evident realization.

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1, baseline=(XXXX.south) ]
\path (0,216);\path (560,0);\draw    ($(current bounding box.center)+(0,0.3em)$) node [anchor=south] (XXXX) {};
%Straight Lines [id:da7397408893276469] 
\draw    (38.67,80.5) -- (334.67,80.5) ;
%Straight Lines [id:da17688600981336555] 
\draw    (37.67,117.5) -- (314.67,116.5) ;
%Straight Lines [id:da9567264788702279] 
\draw    (37.67,155.5) -- (90.67,154.5) ;
%Flowchart: Process [id:dp3559941661194721] 
\draw   (90.67,142.5) -- (116.67,142.5) -- (116.67,169.5) -- (90.67,169.5) -- cycle ;
%Straight Lines [id:da27451132681814205] 
\draw    (103.67,40.5) -- (103.67,142.5) ;
%Straight Lines [id:da42026012714282923] 
\draw    (115.67,155.5) -- (146.67,155.5) ;
%Flowchart: Process [id:dp35222822054449754] 
\draw   (145.67,141.5) -- (171.67,141.5) -- (171.67,168.5) -- (145.67,168.5) -- cycle ;
%Straight Lines [id:da8036844711820179] 
\draw    (171.67,155.5) -- (249.67,155.5) ;
%Flowchart: Process [id:dp11926323599915611] 
\draw   (250.67,140.5) -- (276.67,140.5) -- (276.67,167.5) -- (250.67,167.5) -- cycle ;
%Straight Lines [id:da3111962809283304] 
\draw    (158.67,80.5) -- (158.67,142.5) ;
%Flowchart: Or [id:dp09546044903020046] 
\draw   (199.83,80.25) .. controls (199.83,74.17) and (204.53,69.25) .. (210.33,69.25) .. controls (216.13,69.25) and (220.83,74.17) .. (220.83,80.25) .. controls (220.83,86.33) and (216.13,91.25) .. (210.33,91.25) .. controls (204.53,91.25) and (199.83,86.33) .. (199.83,80.25) -- cycle ; \draw   (199.83,80.25) -- (220.83,80.25) ; \draw   (210.33,69.25) -- (210.33,91.25) ;
%Straight Lines [id:da8712762039236375] 
\draw    (210,43.75) -- (210.33,80.25) ;
%Straight Lines [id:da029591411775552467] 
\draw    (263,116) -- (263.67,140.5) ;
%Flowchart: Or [id:dp7386703963881307] 
\draw   (292.67,80.5) .. controls (292.67,74.42) and (297.37,69.5) .. (303.17,69.5) .. controls (308.97,69.5) and (313.67,74.42) .. (313.67,80.5) .. controls (313.67,86.58) and (308.97,91.5) .. (303.17,91.5) .. controls (297.37,91.5) and (292.67,86.58) .. (292.67,80.5) -- cycle ; \draw   (292.67,80.5) -- (313.67,80.5) ; \draw   (303.17,69.5) -- (303.17,91.5) ;
%Straight Lines [id:da4488792160467461] 
\draw    (303,44.75) -- (303.33,81.25) ;
%Straight Lines [id:da3144490269767424] 
\draw    (277.67,155.5) -- (334.67,155.5) ;
%Straight Lines [id:da409108315676856] 
\draw    (314.67,116.5) -- (337.5,116.5) ;
%Shape: Ellipse [id:dp019878141375235137] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (100,117.5) .. controls (100,114.88) and (101.94,112.75) .. (104.33,112.75) .. controls (106.73,112.75) and (108.67,114.88) .. (108.67,117.5) .. controls (108.67,120.12) and (106.73,122.25) .. (104.33,122.25) .. controls (101.94,122.25) and (100,120.12) .. (100,117.5) -- cycle ;
%Shape: Ellipse [id:dp5115151881818927] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (155,80.75) .. controls (155,78.13) and (156.94,76) .. (159.33,76) .. controls (161.73,76) and (163.67,78.13) .. (163.67,80.75) .. controls (163.67,83.37) and (161.73,85.5) .. (159.33,85.5) .. controls (156.94,85.5) and (155,83.37) .. (155,80.75) -- cycle ;
%Shape: Ellipse [id:dp33480296392000763] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (206,41.75) .. controls (206,39.13) and (207.94,37) .. (210.33,37) .. controls (212.73,37) and (214.67,39.13) .. (214.67,41.75) .. controls (214.67,44.37) and (212.73,46.5) .. (210.33,46.5) .. controls (207.94,46.5) and (206,44.37) .. (206,41.75) -- cycle ;
%Shape: Ellipse [id:dp8043185596483575] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (259,116.75) .. controls (259,114.13) and (260.94,112) .. (263.33,112) .. controls (265.73,112) and (267.67,114.13) .. (267.67,116.75) .. controls (267.67,119.37) and (265.73,121.5) .. (263.33,121.5) .. controls (260.94,121.5) and (259,119.37) .. (259,116.75) -- cycle ;
%Shape: Ellipse [id:dp7855321547442113] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (299,41.75) .. controls (299,39.13) and (300.94,37) .. (303.33,37) .. controls (305.73,37) and (307.67,39.13) .. (307.67,41.75) .. controls (307.67,44.37) and (305.73,46.5) .. (303.33,46.5) .. controls (300.94,46.5) and (299,44.37) .. (299,41.75) -- cycle ;
%Straight Lines [id:da018154455358085686] 
\draw    (39.67,40.5) -- (331.67,41.5) ;
%Shape: Ellipse [id:dp15980648308898693] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (100,41.5) .. controls (100,38.88) and (101.94,36.75) .. (104.33,36.75) .. controls (106.73,36.75) and (108.67,38.88) .. (108.67,41.5) .. controls (108.67,44.12) and (106.73,46.25) .. (104.33,46.25) .. controls (101.94,46.25) and (100,44.12) .. (100,41.5) -- cycle ;
%Shape: Ellipse [id:dp13567476485481245] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (154,116.75) .. controls (154,114.13) and (155.94,112) .. (158.33,112) .. controls (160.73,112) and (162.67,114.13) .. (162.67,116.75) .. controls (162.67,119.37) and (160.73,121.5) .. (158.33,121.5) .. controls (155.94,121.5) and (154,119.37) .. (154,116.75) -- cycle ;
%Straight Lines [id:da296298737344626] 
\draw    (263,80) -- (263.33,116.75) ;
%Shape: Ellipse [id:dp45754197158771626] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (259,80.75) .. controls (259,78.13) and (260.94,76) .. (263.33,76) .. controls (265.73,76) and (267.67,78.13) .. (267.67,80.75) .. controls (267.67,83.37) and (265.73,85.5) .. (263.33,85.5) .. controls (260.94,85.5) and (259,83.37) .. (259,80.75) -- cycle ;
%Straight Lines [id:da15677220995444108] 
\draw    (73.67,107.5) -- (61.67,129.5) ;
% Text Node
\draw (97,146.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {V};
% Text Node
\draw (152,146.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {V};
% Text Node
\draw (252.67,142) node [anchor=north west][inner sep=0.75pt]   [align=left] {V$\displaystyle ^{\dagger }$};
% Text Node
\draw (21,102.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \tilde{c}$};
% Text Node
\draw (21,70.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle b$};
% Text Node
\draw (21,28.5) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle a$};
\end{tikzpicture}

which requires three $(k-1)$-controlled $V$ gates.


\section{Introduction}

The study of quantum algorithms has dramatically transformed in the last few years due to the quantum to classical feedback loop: a fixed depth quantum circuit is adjusted to minimize a cost function.  This approach partially circumvents certain limitations such as variability in pulse timing and can require shorter depth circuits at the cost of outer loop training \cite{harrigan2021quantum,pagano2019quantum, guerreschi2019qaoa,butko2020understanding, Biamonte_2021, campos2020abrupt}. The most studied algorithms in this setting are the Quantum Approximate Optimisation Algorithm (QAOA) \cite{Farhi2014} which was developed to approximate solutions to combinatiorial optimisation problem instances \cite{niu2019optimizing,Farhi2014,lloyd2018quantum,morales2020universality,Zhou2020,wang2020x,Brady2021,Farhi2016,Akshay2020,Farhi2019a,Wauters2020,Claes2021,Zhou} and the variational quantum eigensolver (VQE), developed to find the lowest energy of a Hamiltonian.  The variational approach represents a universal model of quantum computation \cite{Biamonte_2021} and the QAOA gate sequences can, in principle, represent and\todo{EK: any?} quantum circuit \cite{lloyd2018quantum, morales2020universality}.  

The setting of variational quantum computation is that of $n$ qubits: states are represented as vectors in $V_n = [\mathbb{C}^2]^{\otimes n}$.  We are given a non-negative Hamiltonian $P \in \text{herm}_\mathbb{C}(V_n)$ and we seek the lowest eigenvalue of $P$ and/or the circuit settings to prepare the normalized ground vector $\ket{t}\in \arg\min\limits_{\phi \in V_n} \bra{\phi}P\ket{\phi}$.



\section{Background}

Single qubits have evidently been considered in a wide number of settings.  In terms of control theory, the authors \cite{MP19} formulated the control problem to prepare single qubit density matrices in the presence of noise.  Variational quantum algorithms share some motivation with optimal control.  However, the quantum system need not be emulated classically in the case of variational quantum algorithms.  

Mathematically, a pure qubit state $\ket{\psi}$ is a unit vector in $\mathbb{C}^2$ whereas a mixed qubit is a unit trace Hermitian operator on $\mathcal{L}(\mathbb{C^2})$.  For a single qubit, one can express a basis of algebraic invariants.  For a pure state, the only polynomial invariant is the norm: $\braket{U(\psi)}{U(\psi)} = \bra{\psi}U^\dagger U\ket{\psi} = 1$).  For a mixed state $\rho$, there are two invariants.  The trace is invariant as is the determinant
\textcolor{red}{O:Sounds confusing to me since pure state can be also represented with a density matrix. Lets use instead: ket notation and density matrix without reference to pure or mixed cases }

\begin{equation}\label{eqn:det}
    \det \rho = \frac{1}{2}\left( \text{Tr}(\rho^2) - \text{Tr}(\rho)^2\right) = \lambda_- \lambda_+ = \lambda_-(1-\lambda_+)
\end{equation}
where $\lambda_-$, $\lambda_+$ are the non-negative eigenvalues of $\rho$. Any unitary invariant function can be expressed in the polynomial basis $\{\det \rho,  \text{Tr}(\rho)\}$. For example, 
\begin{equation}
    S{\rho} = - \text{Tr} \rho \ln \rho = - \sum_{l\in \{\pm 1\}} \lambda_l \ln \lambda_l
\end{equation}
is expressed as a basis independent function of $\rho$ with \eqref{eqn:det} and 
\begin{equation}
    \lambda_\pm = \frac{1 \pm \sqrt{\text{Tr}(\rho)^2 - 4\det \rho}}{2}. 
\end{equation}

We will now consider the gates that can be made with the Hamiltonian of the single qubit ion system. 

\subsection{Single qubit ion model}

The qubit model of quantum computation relies on the assumption that two level systems can be physically prepared and manipulated. Modeling a qubit from an ion requires two major components. Firstly the ion needs to be trapped and secondly a laser pulse is used to  manipulate the states of the trapped ion. The Hamiltonian for this composite system is:

\begin{equation}\label{ion_hamil}
    H = H_{\text{ion}} +H_{\text{int}} +H_{\text{trap}}.
\end{equation}
The three terms in Eq.~\eqref{ion_hamil} are:
\begin{enumerate}
    \item $H_{\text{ion}} = \sum_n \hbar \omega_n \ketbra{n}{n}$ where $\ket{n}$ represents the internal degree of freedom of the ion.
    \item $H_{\text{int}} = -{\bf d} \cdot {\bf E}$. Here ${\bf d} = \sum_{kl} {\bf d}_{kl} \ketbra{k}{l}$ is the electric dipole operator decomposed in the  and internal degree of freedom of the ion. ${\bf E} = {\boldsymbol{\epsilon}} e^{- i \omega t} + {\boldsymbol{\epsilon}}^* e^{i \omega t}$ is the electric field of the laser.
    \item $H_{\text{trap}} = \hbar \nu (a^\dagger a + \frac{1}{2})$ which describes the motion of the ion in the trap. Here $\nu$ is the oscillation frequency. 
\end{enumerate}

\subsubsection*{Effective two level Hamiltonian} In its simplest form an effective two level ion system disregards the trap Hamiltonian. Thus the system is described solely in terms of the internal degree of freedom. We use the rotating wave approximation to arrive at the effective two level Hamiltonian. The effective Hamiltonian $H_{\text{eff}}$ describing a two level system with basis states $\{ \ket{g}, \ket{e} \}$ is given as:
\begin{align} \label{hwt}
    H_\text{eff} &= -\Delta \ketbra{e}{e} -{\bf d}_{eg} \cdot {\boldsymbol{\epsilon}} \ketbra{e}{g} - {\bf d}_{ge} \cdot {\boldsymbol{\epsilon}}^* \textcolor{red}{\ketbra{g}{e}} \nonumber\\
    &= -\frac{\Delta}{2} \sigma^0 - \operatorname{Re}({\bf d}_{eg} \cdot {\boldsymbol{\epsilon}}) \sigma^1 + \operatorname{Im}({\bf d}_{eg} \cdot {\boldsymbol{\epsilon}}) \sigma^2 -\frac{\Delta}{2} \sigma^3 \nonumber \\
    &=n_0 \sigma^0 + {\bf n} \cdot {\boldsymbol \sigma}.
\end{align}

where $n_0 = -\frac{\Delta}{2}$ and ${\bf n} = (-\operatorname{Re}({\bf d}_{eg} \cdot {\boldsymbol{\epsilon}}), \operatorname{Im}({\bf d}_{eg} \cdot {\boldsymbol{\epsilon}}), -\frac{\Delta}{2})$ \textcolor{red}{and $\sigma$-s are Pauli matrices}. $H_{\text{eff}}$ is written in a rotating frame of reference (transformed with respect to $\omega \ketbra{e}{e}$) and assumes the position of the ion to be fixed at $x = 0$. Here the detuning $\Delta = \omega - \omega_g + \omega_e$ is considered to be small and the AC stark shifts are disregarded. Transitions $\ket{g} \leftrightarrow \ket{e}$ occur when $\omega \sim \omega_e - \omega_g$. The eigenenergies of $H_{\text{eff}}$ are given by $\lambda_\pm = -\frac{\Delta}{2} \pm \sqrt{\frac{\Delta^2}{4}+ |{\bf d}_{eg} \cdot {\boldsymbol{\epsilon}}|^2}$ with the following eigenstates:

\begin{equation}
    \ket{\lambda_\pm} = \frac{1}{\sqrt{|{\bf d}_{eg} \cdot {\boldsymbol{\epsilon}}|^2 + \lambda_\mp^2}}({\bf d}_{eg} \cdot {\boldsymbol{\epsilon}} \ket{e} + \lambda_\mp \ket{g})
\end{equation}
% and 
% \begin{equation}
%     \ket{\lambda_-} = \frac{\sqrt{2} \vert {\bf d}_{eg} \cdot {\boldsymbol{\epsilon}} \vert}{\sqrt{2-\Delta}} \ket{e} - \frac{\sqrt{2-\Delta}}{2\sqrt{2}} \frac{{\bf d}_{eg} \cdot {\boldsymbol{\epsilon}}}{\vert {\bf d}_{eg} \cdot {\boldsymbol{\epsilon}} \vert} \ket{g}.
% \end{equation}

\subsubsection*{Total Hamiltonian}
A more realistic Hamiltonian that describes a two level ion system no longer disregards the trap. Therefore we now deal with both the internal degree of freedom ($\{ \ket{g}, \ket{e} \}$) as well as the motional degree of freedom ($\{\ket{m}\}$) due to the trap Hamiltonian. Thus our new Hilbert space is isomorphic to $\mathbb{C}^\infty \otimes \mathbb{C}^2$ with a basis $\{\ket{m,g}, \ket{m,e}\}_{m=1}^\infty$. This allows for additional transitions in addition to the direct transitions $\ket{m,g} \leftrightarrow \ket{m,e}$ when $\omega \sim (\omega_e - \omega_g)$. The new transitions corresponds to the sideband resonances:
\begin{enumerate}
    \item $\ket{m,g} \leftrightarrow \ket{m-1, e}$ for $\omega \sim (\omega_e - \omega_g - \nu)$
    \item $\ket{m,g} \leftrightarrow \ket{m+1, e}$ for $\omega \sim (\omega_e - \omega_g + \nu)$
\end{enumerate}

The total Hamiltonian that describes this system can be written as
\begin{align}
    H &= \hbar \nu (a^\dagger a + \frac{1}{2}) - \Delta \ketbra{e}{e} - {\bf d}_{eg} \cdot {\boldsymbol{\epsilon}} ( \mathbf{1} +i \eta a +i \eta a^\dagger) \ketbra{e}{g} + h.c. \nonumber \\
    &= \hbar \nu (a^\dagger a + \frac{1}{2}) + n_0 \sigma^0 + {\bf n} \cdot {\boldsymbol \sigma} + \eta (a + a^\dagger) (\operatorname{Im}({\bf d}_{eg} \cdot {\boldsymbol{\epsilon}}) \sigma^1 + \operatorname{Re}({\bf d}_{eg} \cdot {\boldsymbol{\epsilon}}) \sigma^2)
\end{align}
where $n_0, {\bf n}$ are the same as in Eq.~\eqref{hwt}. $H$ is written in a rotating frame of reference (transformed with respect to $\omega \ketbra{e}{e}$) and we assume that the Lamb-Dicke coefficient $\eta = \sqrt{\frac{\hbar k^2}{2 M \nu}} << 1$.
\todo[inline]{JB: Write Hilbert space and basis for QHO. Express the Hamiltonian as a pauli vector, a QHO and then the coupling term.  As we can diagonalize this, we can writs its Green's function and show the side band transitions.}
\subsection{The variational model of quantum computation}

\begin{enumerate}

    \item {\bf Computational task}.  Minimize a cost function defined by a Hamiltonian. 
    
    \item {\bf States}. A list of real parameters $\boldsymbol{\theta}$ determines a circuit to produce $\ket{\psi ( \boldsymbol{\theta} )}$. For a single qubit, any state can be preprared by a variational sequence $\exp{i \theta_2 Y} \exp{i \theta_1 X} \ket{0}$.
    
    \item {\bf Measurements}. Expected values of measurements of Pauli strings, $\boldsymbol{\sigma} = \bigotimes_{j=1}^{n} \sigma_j^{\alpha_{j}}$ for $\alpha_{j} \in \lbrace 0,1,2,3 \rbrace$ are computed for each $\ket{\psi ( \boldsymbol{\theta} )}$: $\mathbb{E}[\boldsymbol{\sigma}] = \bra{\psi ( \boldsymbol{\theta} )} \bigotimes_{j=1}^{n} \sigma_j^{\alpha_{j}} \ket{\psi ( \boldsymbol{\theta} )}$
    
    \item {\bf Compute cost function}. A cost function defined by a weighted sum of expected values is computed for each $\ket{\psi ( \boldsymbol{\theta} )}$.  
    
    \item {\bf Outer-loop optimization}. Classical optimization routines update parameters $\boldsymbol{\theta}\rightarrow \boldsymbol{\theta}_\star$. For example, gradient descent-based methods can be used.
\end{enumerate}

\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{variational.png}
    \caption{The quantum-to-classical iteration process as a block diagram. The cost function is computed classically by considering a weighted sum of expected values calculated on the quantum processor. }
    \label{fig:variational}
\end{figure}

\begin{remark}[Computing the expected value]
The expected value of a sum is a sum of expected values.   
\begin{equation} \label{eqn:convolution}
\bra{\psi}{H}\ket{\psi} = \bra{\psi}{\sum_k h_k\bigotimes_{j=1}^{n} \sigma_j^{\alpha_{j}(k)} }\ket{\psi} = \sum_k h_k \bra{\psi}{\bigotimes_{j=1}^{n} \sigma_j^{\alpha_{j}(k)}}\ket{\psi}
\end{equation}
where $h_k$ is a real number and $\bigotimes_{j=1}^{n} \sigma_j^{\alpha_{j}(k)}$ is a Pauli string for $\alpha_{j} \in \lbrace 0,1,2,3 \rbrace$.  
\end{remark}

\begin{remark}[Iterations]
Given copies of $\ket{\psi}$, measuring $\bigotimes_{j=1}^{n} \sigma_j^{\alpha_{j}(k)}$ repeatedly gives an estimate for each $\bra{\psi}{\bigotimes_{j=1}^{n} \sigma_j^{\alpha_{j}(k)}}\ket{\psi}$ separately.\footnote{While the objective function can be evaluated term-wise, achieving tolerance $\sim\epsilon$ requires $\sim\epsilon^{-2}$ measurements---see Hoeffding's inequality.}  
\end{remark}


\subsection{Single qubit Hamiltonian exact solution}
We express our Hamiltonians as unit Pauli vectors viz.
\begin{equation}
    H = \bf{n}.\bf{\sigma}
\end{equation}
The $l_2$ unit $\mathbb{R^3}$ vector $\bf n$ of the desired form can be canonically expressed as 
\begin{equation}\label{eqn:n}
    \bf{n}(\theta, \phi) = \left(\sin(\theta) \cos(\phi), \sin(\theta) \sin(\phi), \cos(\theta) \right). 
\end{equation}
The eigenvalues of $\bf{n}.\bf{\sigma}$ are $\pm 1$ and the eigenvectors are given as 
\begin{equation}
    \ket{\lambda_+} = \cos \left(\frac{\theta}{2}\right) \ket{0} + \sin \left(\frac{\theta}{2}\right) e^{\imath \phi}\ket{1} 
\end{equation}
and 
\begin{equation}
    \ket{\lambda_-} = \sin \left(\frac{\theta}{2}\right) \ket{0} - \cos \left(\frac{\theta}{2}\right) e^{\imath \phi}\ket{1}. 
\end{equation}

The standard stability lemma \cite{Biamonte_2021} assumes that a non-negative operator has (i) a kernel, (ii) a gap $\Delta$.  We then derive a qubit specific stability lemma.  

\begin{proposition}[Qubit energy to state overlap]
Let $\bf{n}$ be an $l_2$ unit $\mathbb{R^3}$ vector corresponding to Hamiltonian $\bf{n}.\bf{\sigma}$ with normalized ground eigenvector $\ket{\lambda_-}$. Then the expected value relative to $\ket{\omega}$ and the ground state overlap are related as: 
\begin{equation}
    \frac{1-\bra{\omega} \bf{n}.\bf{\sigma} \ket{\omega}}{2} = |\braket{\lambda_-}{\omega}|^2.
\end{equation}
\end{proposition}


\subsection{Collecting data}

In variational quantum computation, we seek to calculate the expected values of Pauli strings.  The measurements are local, single qubit measurements in the $Z$, $X$ or $Y$ basis. 

\begin{remark}[Bernoulli random variables]
Let $\omega_l$ be a sequence of independent identically distributed Bernoulli random variables i.e. $\omega_l$ evaluates to zero with probability $p$ and to one with probability $1-p$. 
\end{remark}

For a given expected value $\bra{\psi}H\ket{\psi}$, and for any sequence  $\omega_l,$ we have 
\begin{equation}\label{eqn:measurementslimit}
    \lim_{k\rightarrow \infty} \frac{\sum_{l=1}^k (-1)^{\omega_l}}{k} = \bra{\psi}H\ket{\psi}. 
\end{equation}

Hoeffding's inequality will be used to bound the convergence of \eqref{eqn:measurementslimit}. 

\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{pics/convergence.eps}
    \caption{Convergence error (blue) versus samples against the Hoeffding inequality (green).  Samples taken from Bernoulli series of binary measurements to form empirical mean.  The ordinate axis is the total samples taken, each point being independently generated data. The tolerance is $\epsilon = 0.05$.  After the samples sizes pass 1,000, the probability of the empirical expected value fluctuating more than $\epsilon$ from the true expected value rapidly approaches zero.  }
    \label{fig:measurement}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{pics/expected_value_convergence_4.eps}
    \caption{Expectation value convergence in the number of shots for a uniformily generated random state and Hamiltonian of the form $\bf{n}.\sigma$. Curves illustrate the standard error $\sqrt{\frac{1-\langle H \rangle^2}{N}}$, where H is $X$, $Y$, or $Z$, and $N$ is the number of shots.}
    \label{fig:my_label}
\end{figure}
A probability bound---also called a concentration inequality---considers the probability of an empirically measured random variable(s) $\mathbb{P}(S)$ to differ from its true mean $\mathbb{E}(S)$.  For example, we seek to determine closed and empirical forms for
\begin{equation}
    \mathbb{P}(S\geq \mathbb{E}(S)+t) 
\end{equation}
and 
\begin{equation}
    \mathbb{P}(S\leq \mathbb{E}(S)-t)
\end{equation}
for some $t\geq 0$.  The most elementary result along these lines is given as: 
\begin{proposition}[Markov's inequality] Let $S$ be a non-negative random variable with expected value $\mathbb{E}(S)$, then $\forall t\geq 0$
\begin{equation}
    \mathbb{P}[S - \mathbb{E}(S)\geq t]\leq \frac{\mathbb{E}(S)}{t}. 
\end{equation}
\end{proposition}

\begin{example}
Use the affine relation to re-scale the expected value and apply the inequality above.  \todo{todo} 
\end{example}

\begin{proposition}[Chebyshev’s inequality] Let $S$ be a random variable with mean $\mathbb{E}(S)$ and variance $\mathbb{V}(S)<\infty$, then $\forall t\geq 0$
\begin{equation}
    \mathbb{P}[S\geq \mathbb{E}(S) + t~\text{or}~S\leq \mathbb{E}(S) - t] \leq \frac{\mathbb{V}(S)}{t^2}. 
\end{equation}
\end{proposition}

\begin{proposition}[Chebyshev inequality for Bernoulli random variables]
Let $S_1, \dots, S_m$ be a sequence of Bernoulli random variables with mean $p$ and let the empirical mean for the sequence be $S=\frac{1}{m} \sum_{l=1}^m S_l$.  Then, 
\begin{equation}
    \mathbb{P}[ |S - p| > \epsilon] \leq \frac{1}{4n\epsilon^2}
\end{equation}
\end{proposition}


\begin{example}
Compare this with the last example.  \todo{todo} 
\end{example}

\begin{proposition}[Hoeffding’s inequality] Let $S_1, \dots, S_m$ be a sequence of independent and identically distributed random variables on $[0, 1]$ with mean $\mathbb{E}(S)$ and empirical mean $S=\frac{1}{m} \sum_{l=1}^m S_l$.  Then, 
\begin{equation}
    \mathbb{P}[ |S - \mathbb{E}(S)| > \epsilon] \leq \delta = 2 \exp[-2 m \epsilon^2]
\end{equation}
\end{proposition}

\begin{proposition}[Hoeffding's bound] Suppose we chose the sample number 
\begin{equation}
    m \geq \frac{1}{2 \epsilon^2} \log \frac{2}{\delta} 
\end{equation}
then with probability at least $1-\delta$ the difference between the empirical mean $S= \frac{1}{m} \sum_{l=1}^m S_l$ and the true mean $\mathbb{E}(S)$ is bounded above by $\epsilon$. 
\end{proposition}

% Rademacher random variable 
% Confidence interval -- true value lies here with some probability 

\begin{proposition}[Hoeffding error] If we draw $m$ samples, then with probability at least $1-\delta$ the difference between the empirical mean $S= \frac{1}{m} \sum_{l=1}^m S_l$ and the true mean $\mathbb{E}(S)$ is at most $\epsilon$ where 
\begin{equation}
    \epsilon \leq \sqrt{\frac{1}{2m} \log \frac{2}{\delta}}. 
\end{equation}

\end{proposition}






\section{Conclusion}



\begin{acknowledgments}
The authors acknowledge support from the project, XXX (Agreement No.~000/00). 
\end{acknowledgments}

% \section{Linear algebra using a trapped ion qubit} 
% Consider the standard matrix inversion problem: 
% \begin{equation}
%     A \ket{x} = \ket{b}
% \end{equation}
% For $A$ and $2\times 2$ matrix and $\ket{x}, \ket{b}$ $2\times 1$ $l_2$ unit vectors.  The objective is to determine $\ket{x}$.  This can be solved in many ways, the standard approach assumes $A^{-1}$ exists, yielding $\ket{x} = A^{-1}\ket{b}$. 

% The solution can also be expressed as an optimisation problem 
% \begin{equation}
%     \max_x \bra{A(x)} P_b \ket{A(x)} 
% \end{equation}
% where the projector $P_b = \ketbra{b}{b}$.\todo{if  $P_b = \bra{b}\ket{b}=1$ }  In this case, we will consider $\ket{\psi(\boldsymbol{\theta})}$ to represent $\ket{x}$.  We then consider the following.  

% Generally we will write 
% \begin{equation}
%     P_b = {\bf b}.{\bf \sigma}
% \end{equation}
% for some choice of ${\bf b}$.  Likewise, let us expand $A$ \todo{Works only if $A$ is Hermitian? If so, $\ket{A(x)}$ is not guaranteed to be of unit length} as 
% \begin{equation}
%     A = {\bf a}.{\bf \sigma} 
% \end{equation}
% in which case, 
% \begin{equation}
%     \max_x \bra{A(x)} P_b \ket{A(x)} = \max_x \bra{A(x)} \sum_l  b_l\sigma^l \ket{A(x)} = \max_x \sum_l b_l \bra{A(x)} \sigma^l \ket{A(x)}
% \end{equation}




\bibliographystyle{unsrt}
\bibliography{references.bib}

\input{appendix_infidelity}

\newpage
\appendix

\section{}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\textwidth]{pics/LRC-1qubit_vqe-error_shots-30runs-2_8192shots-Cobyla-std.pdf}
    \includegraphics[width=0.8\textwidth]{pics/LRC-1qubit_vqe-nfevs_shots-30runs-2_8192shots-Cobyla-std.pdf}
    \caption{Dependence of the difference between the exact ground state energy and that found by VQE (upper) and of the number of function evaluations needed for the COBYLA minimizer to converge (lower) on the number of shots $N_\mathrm{tot}$. The target Hamiltonian is $H = -\sqrt{\frac{1}{6}}X + \sqrt{\frac{2}{6}}Y - \sqrt{\frac{3}{6}}Z$. Blue circles indicate mean values averaged over 30 independent runs. The error bars show the standard errors. On the upper plot, the mean values are well-approximated by the function $f(N_\mathrm{tot})=\frac{2}{3}\frac{1}{\sqrt{N_\mathrm{tot}}}$.}
    \label{fig:error_nfevs-shots}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\textwidth]{pics/LRC-1qubit_vqe-energy_iterations-ibmq_armonk-8192shots-Cobyla.pdf}
    \caption{Energy of the ground state versus the iteration number of the COBYLA minimizer while executing the VQE algorithm on the Armonk quantum chip of IBM. $H = -\sqrt{\frac{1}{6}}X + \sqrt{\frac{2}{6}}Y - \sqrt{\frac{3}{6}}Z$. The solid black line indicates the exact ground state energy.}
    \label{fig:vqe-armonk}
\end{figure}


==> readout_errors_correction.tex <==
\subsection{Correcting readout errors}

Readout of a trapped ion qubit is conducted via detection of the bright state (state $\ket{0}$ in our case) fluorescence. The procedure has a number of instrumental errors associated with the dark state fluorescence, photon detector dark counts, the limited efficiency of radiation collection, and the limited readout time \cite{wolk2015state,bruzewicz2019trapped,christensen2020high}. As a result there is:
\begin{itemize}
    \item a non-unit probability $1 - \varepsilon_{10}$ that the system in the state $\ket{0}$ gives ``0'' result;
    \item a non-zero probability $\varepsilon_{01}$ that the system in the state $\ket{1}$ gives ``0'' result.
\end{itemize}
Thus, the total probability to get ``0'' is $\lambda=p(1 - \varepsilon_{10})+(1-p)\varepsilon_{01}$. Meanwhile, the standard estimator for $p$ is $k/n$, where $k$ is the total number of ``0'' observed. The resulting estimator \eqref{eq:h_of_p} of $\hat{h}_\psi$ is biased:
\begin{equation}
    b=\mathbb{E}(\hat{h}_\psi) - h_\psi = (1-h_\psi)\varepsilon_{01} - (1+h_\psi)\varepsilon_{10}.
\end{equation}
The ideal case when $\varepsilon_{01}, \varepsilon_{10} \rightarrow 0$ gives an unbiased estimator. When the both readout errors are equal to $\varepsilon$ one obtains $b=-2h_\psi\varepsilon$.

However, one can preliminarily estimate $\varepsilon_{01}$ and $\varepsilon_{10}$ \cite{zalivako2021experimental} and build an unbiased estimator \cite{lvovsky2004iterative,schwemmer2015systematic,hou2016error,avosopiants2018non,bantysh2020quantum,ramadhani2021quantum}. For our case the maximum likelihood method gives
\begin{equation}\label{eq:p0_ML}
    \hat{p}_{ML} = \left\{\begin{array}{ll}
         \frac{k/n-\varepsilon_{01}}{1-\varepsilon_{01}-\varepsilon_{10}}, & \text{if }k/n \geq \varepsilon_{01}, \\
         0, & \text{otherwise}.
    \end{array}
    \right.
\end{equation}
Its variance is $g \cdot \mathbb{V}(\hat{p})$ with factor
\begin{equation}\label{eq:var_factor}
    g = \frac{1}{(1-\varepsilon_{01}-\varepsilon_{10})^2}\frac{\lambda(1-\lambda)}{p(1-p)} = 
    \frac{\left[p(1-\varepsilon_{10})+(1-p)\varepsilon_{01}\right]\left[p\varepsilon_{10}+(1-p)(1-\varepsilon_{01})\right]}{p(1-p)(1-\varepsilon_{01}-\varepsilon_{10})^2}
\end{equation}
Given zero readout errors one obtains $g = 1$. Note that the classical infidelity is increased by the same factor when the readout errors are present (see Appendix).

Substituting \eqref{eq:p0_ML} into \eqref{eq:h_of_p} gives an unbiased estimator of Pauli operator expected value. Its variance is $g \cdot \mathbb{V}(\hat{h}_\psi)$. Given $h_\psi=0$ the required sample size is slightly higher than in \eqref{eq:sample_bound}:
\begin{equation}\label{eq:sample_bound_err}
    n = \left(\frac{q_{\alpha/2}}{\delta}\right)^2 \frac{1-(\varepsilon_{01}-\varepsilon_{10})^2}{(1-\varepsilon_{01}-\varepsilon_{10})^2}.
\end{equation}
 
Note that the presented estimator is available only for the given values of $\varepsilon_{01}$ and $\varepsilon_{10}$. One should know them \textit{a-priori} or obtain from the measurements. To make the estimation unbiased, these values must not change significantly during the experiment (the property of statistical stability).


